TEMPEST -- Synthesis Tool for Reactive Systems and Shields in Probabilistic Environments

We present Tempest, a synthesis tool to automatically create correct-by-construction reactive systems and shields from qualitative or quantitative specifications in probabilistic environments. A shield is a special type of reactive system used for run-time enforcement; i.e., a shield enforces a given qualitative or quantitative specification of a running system while interfering with its operation as little as possible. Shields that enforce a qualitative or quantitative specification are called safety-shields or optimal-shields, respectively. Safety-shields can be implemented as pre-shields or as post-shields, optimal-shields are implemented as post-shields. Pre-shields are placed before the system and restrict the choices of the system. Post-shields are implemented after the system and are able to overwrite the system's output. Tempest is based on the probabilistic model checker Storm, adding model checking algorithms for stochastic games with safety and mean-payoff objectives. To the best of our knowledge, Tempest is the only synthesis tool able to solve 2-1/2-player games with mean-payoff objectives without restrictions on the state space. Furthermore, Tempest adds the functionality to synthesize safe and optimal strategies that implement reactive systems and shields

==> examples/optimal_shield_final_format.tex <==
<shieldFileName, Optimal> <<sh>> Rmin=? [ LRA ]

//OUTPUT:
___________________________________________________________________
Optimal-Shield 
                                                          model state:    choice [<value>: (<action {action label})>]:
      2: [!took_detour	& blocked	& move=2	& waiting_time=0	& action=0]    1: (1 {plan2_Dev})
      3: [!took_detour	& blocked	& move=2	& waiting_time=0	& action=1]    1: (0 {plan2})
     15: [!took_detour	& blocked	& move=2	& waiting_time=1	& action=0]    1: (1 {plan2_Dev})


==> examples/postsafety_final_format.tex <==
<shieldFileName, PostSafety, gamma=0.5> Pmax=? [ G<=14 !"crash" ]

//OUTPUT: ___ gehören zum output!
___________________________________________________________________
Post-Safety-Shield with absolute comparison (gamma = 0.5):
                                model state:    correction [<action> {action label}: <corrected action> {corrected action label}]:
     0: [move=0	& x1=0	& y1=0	& x2=4	& y2=4]    0 {e1}: 0 {e1};    1 {s1}: 1 {s1}
     3: [move=0	& x1=1	& y1=0	& x2=3	& y2=4]    0 {e1}: 0 {e1};    1 {w1}: 1 {w1}
     4: [move=0	& x1=1	& y1=0	& x2=4	& y2=4]    0 {e1}: 0 {e1};    1 {w1}: 1 {w1}
    23: [move=0	& x1=2	& y1=0	& x2=4	& y2=3]    0 {e1}: 0 {e1};    1 {w1}: 1 {w1};    2 {s1}: 2 {s1}


==> examples/presafety_final_format.tex <==
<shieldFileName, PreSafety, lambda=0.5> Pmax=? [ G<=14 !"crash" ]

//OUTPUT:
___________________________________________________________________
Pre-Safety-Shield with relative comparison (lambda = 0.5):
                                model state:    choice(s) [<value>: (<action {action label})>]:
     0: [move=0	& x1=0	& y1=0	& x2=4	& y2=4]    1: (0 {e1});    1: (1 {s1})
     3: [move=0	& x1=1	& y1=0	& x2=3	& y2=4]    1: (0 {e1});    1: (1 {w1})
     4: [move=0	& x1=1	& y1=0	& x2=4	& y2=4]    1: (0 {e1});    1: (1 {w1})
     5: [move=0	& x1=1	& y1=0	& x2=4	& y2=3]    1: (0 {e1});    1: (1 {w1})
     6: [move=0	& x1=0	& y1=1	& x2=3	& y2=4]    1: (0 {n1});    1: (1 {s1})
     7: [move=0	& x1=0	& y1=1	& x2=4	& y2=4]    1: (0 {n1});    1: (1 {s1})
     8: [move=0	& x1=0	& y1=1	& x2=4	& y2=3]    1: (0 {n1});    1: (1 {s1})
    18: [move=0	& x1=2	& y1=0	& x2=4	& y2=4]    1: (0 {e1});    1: (1 {w1});    1: (2 {s1})

==> examples/storm_scheduler_aka_controller.tex <==
___________________________________________________________________
Fully defined memoryless deterministic scheduler:
                                               model state:    choice(s)
       0: [!picked_up	& move=0	& x1=4	& y1=0	& x2=4	& y2=0]    1 {s1}
       1: [!picked_up	& move=1	& x1=3	& y1=0	& x2=4	& y2=0]    0 {w2}
       2: [!picked_up	& move=1	& x1=4	& y1=1	& x2=4	& y2=0]    1 {s2}
       3: [!picked_up	& move=0	& x1=3	& y1=0	& x2=3	& y2=0]    1 {w1}


==> examples/warehouse_adv_with_stuck_prob.tex <==
// modeltype
smg

player shieldedRobot
  [e1], [w1], [n1], [s1]
endplayer

player adverseryRobot
  [e2], [w2], [n2], [s2]//, [stay2]
endplayer

// 5x5 grid
const int width = 4;
const int height = 4;

const int xmin = 0;
const int xmax = width;
const int ymin = 0;
const int ymax = height;

// probabilty to get stuck
const double stuckProp = 1/3;
const double notstuckProp = 1 - stuckProp;

global move : [0..1] init 0;

formula robot1BetweenShelves = !(y1=0 | y1=height);
formula robot2BetweenShelves = !(y2=0 | y2=height);
formula robot1AboveShelves = mod(x1, 2) = 1;
formula robot1BelowShelves = mod(x1, 2) = 1;
formula robot2AboveShelves = mod(x2, 2) = 1;
formula robot2BelowShelves = mod(x2, 2) = 1;

//II:

//__F__
//_x_x_R -> 2/3
//_x_xR  -> 1/3
//_x_x_
//_____

//player shieldedRobot
//player adverseryRobot (with prob of being stuck one time step)

label "crash" = x1=x2 & y1=y2;

module robot1
  x1 : [0..width] init 0;
  y1 : [0..height] init 0;

  [e1]    move=0 & x1<xmax & !robot1BetweenShelves -> (x1'=x1+1) & (move'=1);
  [w1]    move=0 & x1>0    & !robot1BetweenShelves -> (x1'=x1-1) & (move'=1);

  [n1]    move=0 & y1>0    & !robot1BelowShelves -> (y1'=y1-1) & (move'=1);
  [s1]    move=0 & y1<ymax & !robot1AboveShelves -> (y1'=y1+1) & (move'=1);
endmodule

module robot2
  x2 : [0..width] init width;
  y2 : [0..height] init height;

  [e2]    move=1 & x2<xmax & !robot2BetweenShelves -> notstuckProp : (x2'=x2+1) & (move'=0) + stuckProp : (move'=0);
  [w2]    move=1 & x2>0    & !robot2BetweenShelves -> notstuckProp : (x2'=x2-1) & (move'=0) + stuckProp : (move'=0);

  [n2]    move=1 & y2>0    & !robot2BelowShelves -> notstuckProp : (y2'=y2-1) & (move'=0) + stuckProp : (move'=0);
  [s2]    move=1 & y2<ymax & !robot2AboveShelves -> notstuckProp : (y2'=y2+1) & (move'=0) + stuckProp : (move'=0);

  //[stay2] move=1 & true -> (move'=0);
endmodule

==> robot_grid.tex <==
\subsection{Robot Capture the Flag}\label{sec:grid_robot}

This experiment features two robots competing over resources in an $NxN$-grid where they are allowed to move in any given direction. They start at two diagonally opposit corners of the grid and their objectives are to get resources, say fuel, from the other robots starting corner. We synthesise \ldots


\begin{tikzpicture}
\begin{axis}[
view={212}{10},
%%width=\axisdefaultwidth,
%height=5cm,
xlabel={$N$},
xmin=3, xmax=12,
ylabel={$P_{failure}$},
%ymin=1e-1, ymax=1e1,
ymin=0, ymax=0.5,
zlabel={$mean fuel level$},
zmin=1e-2, zmax=0.7,
%ymode=log,
zmode=log,
%ztick
]

\addplot3 [surf
] coordinates {

  (3,0,0.1109) (3,0.05,0.1024) (3,0.1,0.0986) (3,0.25,0.0892) (3,0.5,0.0509)

  (4,0,0.1664) (4,0.05,0.1804) (4,0.1,0.1897) (4,0.25,0.1956) (4,0.5,0.1697)

  (5,0,0.3204) (5,0.05,0.3095) (5,0.1,0.3015) (5,0.25,0.2847) (5,0.5,0.2583)

  (6,0,0.3877) (6,0.05,0.3775) (6,0.1,0.3722) (6,0.25,0.3557) (6,0.5,0.3097)

  (8,0,0.4485) (8,0.05,0.4477) (8,0.1,0.4494) (8,0.25,0.4202) (8,0.5,0.3639)

  (10,0,0.4872) (10,0.05,0.4883) (10,0.1,0.4881) (10,0.25,0.4543) (10,0.5,0.3926)

  (12,0,0.5139) (12,0.05,0.5186) (12,0.1,0.5129) (12,0.25,0.4785) (12,0.5,0.4196)
};
\end{axis}
\end{tikzpicture}
\label{fig:robot_grid_lra}

\begin{tikzpicture}
\begin{axis}
\addplot[color=blue,
    mark=square]
coordinates {(0,0.1109) (0.05,0.1024) (0.1,0.0986) (0.25,0.0892) (0.5,0.0509)};
\addplot[color=olive,
    mark=x,
    ]
coordinates {(0,0.1664) (0.05,0.1804) (0.1,0.1897) (0.25,0.1956) (0.5,0.1697)};
\addplot[color=green,
    mark=square,
    ]
coordinates {(0,0.3204) (0.05,0.3095) (0.1,0.3015) (0.25,0.2847) (0.5,0.2583)};
\addplot[color=magenta,
    mark=x,
    ]
coordinates { (0,0.3877) (0.05,0.3775) (0.1,0.3722) (0.25,0.3557) (0.5,0.3097)};
\addplot[color=orange,
    mark=square,
    ]
coordinates {(0,0.4485) (0.05,0.4477) (0.1,0.4494) (0.25,0.4202) (0.5,0.3639)};
\addplot[color=violet,
    mark=x,
    ]
coordinates { (0,0.4872) (0.05,0.4883) (0.1,0.4881) (0.25,0.4543) (0.5,0.3926)};
\addplot[color=red,
    mark=x,
    ]
coordinates {(0,0.5139) (0.05,0.5186) (0.1,0.5129) (0.25,0.4785) (0.5,0.4196)};
\end{axis}
\end{tikzpicture}


==> virus_network.tex <==
\subsection{Network Virus Infection}\label{sec:virus}

In this experiment we study the behaviour of a computer virus spreading through a network of personal computers. Two agents are attacking or defending the nodes of this network, respectively. The network is modelled as a grid of $m X n$ neighbouring nodes each connected to at most four adjacent nodes, two being connected horizontally, the other two vertically. The experiment starts with the node in the top left corner being infected with the computer virus. The attacking agents goal is to infect as many of the networks nodes as possible. An attack is subject to a certain probability of success $a$, which may be viewed as the probability of breaching a target computers firewall. Once a node has been successfully infected it may be used by the attacking agent to infect other nodes. The defending agents goal is to remove the virus from an infected node. The node which is infected at the beginning of the game \textit{may not be cleaned of the virus}. We model the detection rate of an infected nodes virus by the defending agent with probability $c$. The defending agents goal is therefore to minimize the amount of infected node, which may be expressed by the following: $<<defender>> R\{"infections"\}min=? [ S ]$, where the reward structure "infections" is the sum of all infected nodes. \\


We vary the success rates of both the attacking and defending agents and present the results in \ref{fig:virus_lra}

\begin{tikzpicture}
\begin{axis}
\addplot[color=blue,
    mark=square]
coordinates {(2,1.998)     (4,3.998) (6,5.996) (9,8.993) (12,11.99)};
\addplot[color=olive,
    mark=x,
    ]
coordinates {(2,1.528)   (4,2.712)   (6,4.051)   (9,6.316)   (12,8.828)};
\addplot[color=green,
    mark=square,
    ]
coordinates {(2,1.5)     (4,2.498)   (6,3.495)   (9,4.99)    (12,6.484)};
\addplot[color=magenta,
    mark=x,
    ]
coordinates {(2,1.474)  (4,2.284)  (6,2.938)  (9,3.662)  (12,4.138)};
\addplot[color=orange,
    mark=square,
    ]
coordinates {(2,1.396) (4,1.782) (6,1.935) (9,1.991) (12,1.998)};
\addplot[color=violet,
    mark=x,
    ]
coordinates {(2,1.061) (4,1.063) (6,1.063) (9,1.063) (12,1.063)};
\end{axis}
\end{tikzpicture}
\label{fig:virus_lra}

As expected we \ldots

